The Case for Learning Application Behavior to Improve Hardware Energy Efficiency

Computer applications are continuously evolving. However, significant knowledge can be harvested from a set of applications and applied in the context of unknown applications. In this paper, we propose to use the harvested knowledge to tune hardware configurations. The goal of such tuning is to maximize hardware efficiency (i.e., maximize an applications performance while minimizing the energy consumption). Our proposed approach, called FORECASTER, uses a deep learning model to learn what configuration of hardware resources provides the optimal energy efficiency for a certain behavior of an application. During the execution of an unseen application, the model uses the learned knowledge to reconfigure hardware resources in order to maximize energy efficiency. We have provided a detailed design and implementation of FORECASTER and compared its performance against a prior state-of-the-art hardware reconfiguration approach. Our results show that FORECASTER can save as much as 18.4% system power over the baseline set up with all resources. On average, FORECASTER saves 16% system power over the baseline setup while sacrificing less than 0.01% of overall performance. Compared to the prior scheme, FORECASTER increases power savings by 7%.

==> rel.tex <==
Tarsa et al.~\cite{tarsa19} propose a lightweight ML framework that can be distributed through firmware updates to the microcontroller for post-silicon CPUs. The ML model is first trained offline with a diverse collection of applications to avoid statistical blind spots. During execution, the CPU dynamically sets the issue width of a clustered hardware component while clock-gating unused resources based on the prediction of the ML model.

Pan et al.~\cite{mlrl} present a multi-level reinforcement learning framework (MLRL) to address the scalability issue of the dynamic power management in multi-core processors. MLRL effective reduce the exponential decision process into a linear problem by exploiting the hierarchical paradigm. In MLRL, core states and Q-values are propagated from the bottom to the top of the tree structure, then decisions are propagated back down the tree, providing an efficient control mechanism.

Ravi et al.~\cite{charstar} propose CHARSTAR, a clock tree aware resource optimizing mechanism. CHARSTAR incorporates a multi-layer perceptron with one hidden layer to predict the optimal configuration in each execution phase. The neural network takes into account the clock hierarchy and the topology overhead in order to improve the power savings. However, the offline trained model may soon be obsolete for future unmet programs. Secondly, CHARSTAR only works for single-threaded programs, and a multi-threaded version may cause a super-linearly increase in the size of the neural network model. 
